A Case Study on Noise Resilient Operator Selection in Adaptive Variational Quantum Algorithms

Hardware noise has been shown to significantly impact the accuracy of ADAPT-VQE, a ground state preparation algorithm. While previous work has studied the impact of noise on its parameter optimization step, its impact on the critical operator selection step remains comparatively unexplored. In this work, we examine the impact of a variety of noise channels on this step, using a linear H$_3$ molecule as a test case. We show that, despite the selection criterion's natural resilience to some noise, both coherent and incoherent noise can prevent convergence for sufficiently high noise rates. We employ quantum error mitigation techniques--dynamical decoupling, zero noise extrapolation, and Pauli twirling--and show that when combined appropriately, these techniques are capable of restoring a successful convergence profile. Our results highlight how error mitigation can improve the performance of ADAPT-VQE and enable convergence in the presence of hardware noise, offering valuable insights into the implementation of the algorithm on near-term quantum hardware.

==> intro-paragraph.tex <==
Although previous works have studied the impact of noise and error mitigation on various algorithms, more research is necessary to better understand this topic. In particular, coherent noise is often ignored in simplified noise models. While it is known that Pauli Twirling (PT) can turn coherent errors into stochastic noise \cite{winick_concepts_2022, wallman_noise_2016}, the best complement for this method remains an open question---certain sources recommend DD as an effective complement of PT, while others opt for ZNE instead \cite{dalton_quantifying_2024, kurita_synergetic_2023}. In the particular case of ADAPT-VQE, neither combination has been applied to combat coherent noise, as previous work has considered simplified noise models with a notable absence of coherent noise \cite{dalton_quantifying_2024}. Additionally, previous work has focused on the impact of noise on the energy evaluation and on the optimization of ADAPT-VQE and VQE in general. In contrast, the impact of noise on the ADAPT-VQE operator selection has mostly been ignored in previous studies. This study aims to address this research question by diving into the impact of noise on operator selection and studying whether EM techniques succeed in mitigating this impact. We find that both coherent and incoherent noise can significantly alter the distribution of the gradients; incoherent noise can be especially harmful, as it can wash out the differences and make it difficult to resolve the highest gradient. We show that error mitigation strategies are effective at preventing this; for incoherent noise, DD+ZNE was consistently strongest; for coherent noise, PT paired with ZNE, DD, or both—PT+ZNE, PT+DD, PT+DD+ZNE—performed best.
